Contrastive View Design Strategies to Enhance Robustness to Domain Shifts in Downstream Object Detection

Contrastive learning has emerged as a competitive pretraining method for object detection. Despite this progress, there has been minimal investigation into the robustness of contrastively pretrained detectors when faced with domain shifts. To address this gap, we conduct an empirical study of contrastive learning and out-of-domain object detection, studying how contrastive view design affects robustness. In particular, we perform a case study of the detection-focused pretext task Instance Localization (InsLoc) and propose strategies to augment views and enhance robustness in appearance-shifted and context-shifted scenarios. Amongst these strategies, we propose changes to cropping such as altering the percentage used, adding IoU constraints, and integrating saliency based object priors. We also explore the addition of shortcut-reducing augmentations such as Poisson blending, texture flattening, and elastic deformation. We benchmark these strategies on abstract, weather, and context domain shifts and illustrate robust ways to combine them, in both pretraining on single-object and multi-object image datasets. Overall, our results and insights show how to ensure robustness through the choice of views in contrastive learning.

==> figures/approach_fig.tex <==
   \begin{figure*}[h!]
        
        \begin{center}
            \includegraphics[scale=0.225]{images/method3p0.png}
        \end{center}
        \vspace{-18pt}
        \caption{Our approach. We construct object-focused views in contrastive pretraining to improve downstream robustness to various domain shifts in object detection. Such views can be used to enhance state-of-the-art detection-focused pretext tasks (\eg InsLoc). }
        \label{fig:method}
    \end{figure*}

==> figures/crop_compare_fig.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[scale=0.34]{images/crops_ex.PNG}
    \caption{\textbf{DeepUSPS Tightened Crops \textcolor{Blue}{(Blue)} vs. ContraCAM-Based OA-Crops \cite{mo2021object} \textcolor{Red}{(Red)}.} Note that the DeepUSPS-based crops are tighter to objects (cols 1/4), while not significantly cropping away global object shape or distinctive parts (cols 2/3).  }
    \label{crop_compare_fig}
\end{figure}

==> tables/coco_main.tex <==
        \begin{table*}[t]
            \begin{center}
                \renewcommand{\arraystretch}{1}
                \begin{tabular}{|c|c|c|gg|cc|cc|}
                    \hline
                        \textbf{Method} & \textbf{Crop\%} &
                        \textbf{Aug} &  \multicolumn{2}{c|}{\textbf{COCO}} & \multicolumn{2}{c|}{\textbf{UnRel}} & \multicolumn{2}{c|}{\textbf{COCO-Weather}} \\
                        & & & \multicolumn{1}{c}{AP} & \multicolumn{1}{c|}{AP$_{50}$} & AP & AP$_{50}$ & \multicolumn{1}{c}{AP} & \multicolumn{1}{c|}{AP$_{50}$}  \\
                        \hline\hline
                        InsLoc  
                        & *20-100 & Default & 14.59 & 26.16 & 11.33 & 22.60 & 5.75 & 10.53  \\
                        \cite{yang2021instance} & 70-100 & Default  & 13.91 & 24.70 & 10.74 & 20.87 & 5.34 & 9.56  \\
                        & 20-100 & TextFlatNS & 14.99 & 26.94 & 11.79 & 23.00 & \underline{6.28} & \underline{11.37} \\
                        & 70-100 & TextFlatNS & \underline{15.39} & \underline{27.12} & \underline{11.86} & \underline{23.03} & \underline{6.28} & 11.25 \\
                        \hline
                        InsLoc + CAST-Based Crops  & *20-100 & Default & 14.92 & 26.70 & 11.71 & 22.36 & 5.77 & 10.58 \\
                       \cite{selvaraju2021casting}  & 20-100 & TextFlatNS & \underline{14.97} & \underline{26.94} & \underline{12.02} & \underline{23.59} & \underline{6.29}  & \underline{11.56}  \\
                        \hline
                        InsLoc + OA-Crop  & *8-100 & Default & 14.23 & 25.55 & 11.80 & 23.10 & 5.38 & 9.82 \\
                        \cite{mo2021object} & 70-100 & Default & 13.77 & 24.53 & 10.61 & 20.40 & 5.31 & 9.65  \\
                        & 8-100 & TextFlatNS & 14.60 & 26.35 & 10.98 & 22.08 & 6.16  & 11.31  \\
                        & 70-100 & TextFlatNS& \underline{15.28} & \underline{27.07} & \underline{11.87} & \underline{23.13} & \underline{6.45} & \underline{11.55} \\
                        \hline
                        InsLoc + DeepUSPS Tightened Crops & 8-100 & Default & 15.61 & 27.76 & 12.81 & 24.59 & 6.74 & 12.20 \\
                        & 20-100 & Default & 16.00 & 28.39 & 13.75 & 26.11 & 6.87  & 12.33  \\
                        & 70-100 & Default & 14.45 & 25.46 & 12.00 & 22.66 & 5.99 & 10.67  \\
                        & 8-100 & TextFlatNS & 15.97 & 28.44 & \underline{\textbf{13.85}} & \underline{\textbf{27.31}}  & 6.76 & 12.27 \\
                        & 20-100 & TextFlatNS & 16.02 & 28.66 & 13.18 & 24.93 & 6.64 & 12.12 \\
                        & 70-100 & TextFlatNS & \underline{\textbf{16.45}} & \underline{\textbf{28.74}} & 13.57 & 25.71 & \underline{\textbf{6.98}} & \underline{\textbf{12.44}}  \\
                        \hline
                \end{tabular}
            \end{center}
            \caption{Our object-focused cropping approach versus InsLoc \cite{yang2021instance}, CAST-Based Crops \cite{selvaraju2021casting}, and OA-Crop \cite{mo2021object} baselines, \textbf{under various augmentation settings}. Models are pretrained for 200 epochs on COCO, finetuned end-to-end on \textbf{COCO} with \textbf{24k schedule}, and evaluated on COCO, UnRel, and COCO-Weather. TextFlatNS=texture flattening of non-salient image regions. Underlined entries represent the best per method, while bold entries represent the best overall. An asterisk (*) denotes the strategy proposed in each original paper. }
            \label{main_coco_24k}
        \end{table*}

==> tables/imagenet.tex <==
\begin{table}
    \begin{center}
        \renewcommand{\arraystretch}{1}
        \begin{tabular}{|c|c|g|c|c|}
            \hline
                \textbf{Method} & \textbf{Crop} & \multicolumn{1}{c|}{\textbf{VOC}} & \multicolumn{1}{c|}{\textbf{Abstract}} & \multicolumn{1}{c|}{\textbf{VOCW}} \\
                & \textbf{\%} & \multicolumn{1}{c|}{AP} & AP & AP \\
                \hline\hline
                InsLoc & 20-100 & 38.91 & 10.84 & 16.66 \\
                \hline
                InsLoc & 70-100 & 38.01 & 11.19 & 16.95 \\
                \hline
                InsLoc + TF & 70-100 & \textbf{40.45} & \textbf{13.57} & \textbf{19.60} \\
                \hline
        \end{tabular}
    \end{center}
    \caption{Results from InsLoc views with altered crop \% and full image texture flattening (TF) when pretraining on 50k sample ImageNet subset (200 epochs) and finetuning on VOC (24k schedule).}
    \label{imagenet}
    \vspace{-7pt}
\end{table}
